Local non-Bayesian social learning with stubborn agents

We study a social learning model in which agents iteratively update their beliefs about the true state of the world using private signals and the beliefs of other agents in a non-Bayesian manner. Some agents are stubborn, meaning they attempt to convince others of an erroneous true state (modeling fake news). We show that while agents learn the true state on short timescales, they "forget" it and believe the erroneous state to be true on longer timescales. Using these results, we devise strategies for seeding stubborn agents so as to disrupt learning, which outperform intuitive heuristics and give novel insights regarding vulnerabilities in social learning.

==> experimentDetails.tex <==
\section{Experimental details} \label{appExpDetails}

%\subsection{Section \ref{secSecondResult} experiment}

The basic workflow of the experiment in Section \ref{secSecondResult} proceeded as follows:
\begin{itemize}
\item Choose a sequence of time horizons $T_n$ that increase linearly, then set $n$ accordingly.
\item Realize the degrees $\{ d_{out}(i) , d_{in}^A(i) , d_{in}^B(i) \}_{i \in [n]}$ after selecting $n$.
\item Define the empirical distributions $f_n, f_n^*$ using the degrees as in \eqref{eqEmpDist}.
\item Evaluate quantity of interest $\E [ \hat{\vartheta}_{T_n}(\phi) | \T ]$ empirically via \eqref{eqMeanTreeBeliefGivenTree} using $f_n, f_n^*$.
\end{itemize}
We repeated this experiment 400 times to obtain 400 samples of $\E [ \hat{\vartheta}_{T_n}(\phi) | \T ]$; the plots in Figure \ref{figSecThmStats} show empirical means and variances across these 400 samples. We used the following parameters:
\begin{itemize}
\item We set $\eta = 0.9$ to emphasize the effect of the network.
\item We let $d_{in}^A(i) = 1 + \textrm{Poisson}(\lambda_A-1)\ \forall\ i \in [n]$, so that $\E [ d_{in}^A(i) ] = \lambda_A$; we choose $\lambda_A$ independent of $n$ so that $\E [ d_{in}^A(i) ] = O(1)$, as required by \ref{assGraphDegSeq}. In particular, we choose $\lambda_A = 2.1$.
\item After realizing $\{ d_{in}^A(i) \}_{i \in [n]}$, we assign one outgoing edge to each $i \in [n]$, then assign each of the remaining $\sum_{i \in [A]} d_{in}^A(i) - n$ outgoing edges independently and uniformly at random. Note that this implies $d_{in}^A(i), d_{out}(i) > 0$ and $\sum_{i \in [n]} d_{in}^A(i) = \sum_{i \in [n]} d_{out}(i)$, as required by \eqref{eqDegSeqBasicAss}.
\item We let $d_{in}^B(i) = \textrm{Poisson}(\lambda_B)$, with $\lambda_B = \lambda_A (1-p_n) / p_n$, so that
\begin{equation}
\E d_{in}^A(i) / ( \E d_{in}^A(i) + \E d_{in}^B(i) )= \lambda_A / ( \lambda_A+\lambda_B) = 1 / ( 1 - (1-p_n)/p_n ) = p_n .
\end{equation}
(This is not precisely what we desire, since \ref{assBranchDegSeq} assumes $p_n \approx \tilde{p}_n = \E_n [ \frac{d_{in}^A(v^*)}{  d_{in}^A(v^*) + d_{in}^B(v^*) } ]$ for $v^*$ sampled proportional to out-degree; however, as shown in the second plot in Figure \ref{figSecThmStats}, this empirically yields distinct cases rates of convergence for $(1-p_n) \rightarrow 0$.)
\item We compare four cases of $p_n$: $p_n = p$ and $p_n =  1 - c_i T_n^{(-i+1)/2}$ for $i \in \{2,3,4\}$, with $p$ and $c_i$ independent of $n$. Note that the three latter cases satisfy
\begin{equation}
(1-p_n)  \propto T_n^{(-i+1)/2} \in \left\{  T_n^{-1/2}  , T_n^{-1} ,  T_n^{-3/2} \right\} ,
\end{equation}
as shown in Figure \ref{figSecThmStats}. Here $p$ and $c_i$ were chosen via trial-and-error so that all four cases behaved roughly the same at the smallest value of $n$ (as in Figure \ref{figSecThmStats}). In particular, we chose
\begin{equation}
p = 0.9, \quad c_2 = 1.3, \quad c_3 = 1.9, \quad c_4 = 2.7 .
\end{equation}
\item We let $T_n \in \{2,3,\ldots,11\}$; here the minimum of 2 was chosen since $T_n = 1$ is a trivial case and the maximum of 11 was chosen due to computational limitations.
\item Given $T_n$, we let $n = \lceil \lambda_A^{2 T_n} \rceil$. Note that this implies $T_n \approx ( \log n ) / ( 2 \log \lambda_A )$, roughly the upper bound in \ref{assGraphHorizon}. With our choice of $T_n$ and $\lambda_A$, $n$ ranged from 20 to (roughly) 12 million.
\end{itemize}
In addition to the summary statistics shown in Figure \ref{figSecThmStats}, we also show histograms of error term $| \E [ \hat{\vartheta}_{T_n}(\phi) | \T ] - L(p_n) |$ across the 400 trials in Figure \ref{figSecThmPmfs}. As discussed in Section \ref{secSecondResult}, this term must converge to zero (in probability) at a sufficiently fast rate to prove Theorem \ref{thmSec}. In Figure \ref{figSecThmPmfs}, these histograms appear to converge quickly to a point mass at zero in the case $p_n \rightarrow p < 1$; in other cases, such behavior does \textit{not} occur, further suggesting a fundamental difference between the cases.

Figure \ref{fig_timeVsBelMore} shows an analogue of Figure \ref{fig_timeVsBel} with budget $b_n = \lceil \tilde{b} |E_n| \rceil$ for each $\tilde{b} \in \{ \frac{1}{1600} ,\frac{1}{800} , \frac{1}{200} , \frac{1}{100}  \}$.

\begin{figure}
\includegraphics[width=5.4in]{pmfs}
\caption{Histograms of 400 samples of the error term $| \E [ \hat{\vartheta}_{T_n}(\phi) | \T ] - L(p_n) |$. When $p_n \rightarrow p < 1$, the histogram appears to decay quickly to a point mass on zero; in other cases, this does not occur.} \label{figSecThmPmfs}
\end{figure}

%\subsection{Section \ref{secEmpirical} experiments} \label{appRealExpDetails}

\begin{figure}
\centering
\begin{subfigure}{\textwidth}
\centering \includegraphics[height=1.6in]{timeVsBel100} \caption{$\tilde{b} = 1/100$}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering \includegraphics[height=1.6in]{timeVsBel200}  \caption{$\tilde{b} = 1/200$}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering \includegraphics[height=1.6in]{timeVsBel800}  \caption{$\tilde{b} = 1/800$}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering \includegraphics[height=1.6in]{timeVsBel1600}  \caption{$\tilde{b} = 1/1600$}
\end{subfigure}
\caption{Varying budget for Figure \ref{fig_timeVsBel} experiment.} \label{fig_timeVsBelMore}
\end{figure}














